Initial Limit Datalog: a New Extensible Class of Decidable Constrained Horn Clauses

We present initial limit Datalog, a new extensible class of constrained Horn clauses for which the satisfiability problem is decidable. The class may be viewed as a generalisation to higher-order logic (with a simple restriction on types) of the first-order language limit Datalog$_Z$ (a fragment of Datalog modulo linear integer arithmetic), but can be instantiated with any suitable background theory. For example, the fragment is decidable over any countable well-quasi-order with a decidable first-order theory, such as natural number vectors under componentwise linear arithmetic, and words of a bounded, context-free language ordered by the subword relation. Formulas of initial limit Datalog have the property that, under some assumptions on the background theory, their satisfiability can be witnessed by a new kind of term model which we call entwined structures. Whilst the set of all models is typically uncountable, the set of all entwined structures is recursively enumerable, and model checking is decidable.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> IEEEtran/tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> lcs.tex <==
%!TEX root = main.tex


\subsection{Lossy Channel Systems}

\lo{
A LCS is a tuple $(Q, M, C, \Delta)$ where $Q$ is a finite set of (control) locations, $M$ is a finite message alphabet, $C$ is a finite set of channels, and $\Delta \subseteq Q \times C \times \set{!, ?} \times M \times Q$ is a finite set of transition rules, with typical elements denoted $\delta$.

A configuration of a LCS with $l$ channels is a pair $(q, \overline u)$ where $q \in Q$ is the current location, and $\overline u \in (M^\ast)^l$ is the channel contents.

Suppose $\sigma = (q, u_1, \ldots, u_l)$ and $\sigma' = (q', u_1', \ldots, u_l')$ are configurations. 
There is a transition from $\sigma$ to $\sigma'$ via rule $\delta \in \Delta$ when
\begin{itemize}
\item[1.] \emph{Read step}: $\delta$ is a reading rule $(q, c_i, ?, a, q')$ and $u_i = a \, u_i'$, while $u_j = u_j'$ for $j \not= i$, or
\item[2.] \emph{Write step}: $\delta$ is a writing rule $(q, c_i, !, a, q')$ and $u_i' = u_i \, a$, while $u_j = u_j'$ for $j \not= i$, or
\item[3.] \emph{Loss step}: $\delta$ is a writing rule $(q, c_i, ?, a, q')$ and $u_j = u_j'$ for all $j$.
\end{itemize}
Thus a message can be lost (case 3) during a step attempting to write to a channel.
However messages in a channel cannot be lost; they can only be removed by reading steps.

There are various ways by which messages in a LCS can be lost. This method, called \emph{write-lossy} \cite{DBLP:conf/lics/ChambartS08}, is the most convenient for technical development, and is equivalent to other standard notions of lossy steps.

It follows that the clauses that define reachability can be simplified as follows:
\begin{align*}
	R\; q\; \bar{c} & \impliedby R\; q'\; \bar{c'} \land a\cdot c_{n+1} = c_i \\ %reading
	R\; q\; \bar{c} & \impliedby R\; q'\; \bar{c'} \land c_{n+1}= c_i\cdot a \\ %writing
	R\; q\; \bar{c} & \impliedby R\; q'\; \bar{c} \\ %loss step
	R\; \bar{q_f}\; \bar{c} & \impliedby \mathsf{true} %terminal
\end{align*}
where 
% $$q'_j = \begin{cases}
% 	q_j \mathrm{\ if\ } j\ne k\\
% 	q' \mathrm{\ if\ } j = k
% \end{cases}$$
$$c'_j = \begin{cases}
	c_j \mathrm{\ if\ } j\ne i\\
	c_{n+1} \mathrm{\ if\ } j = i
\end{cases}$$
}

\tcb{It would be possible to claim that the clauses are a formal definition of lossy channel systems, so we don't need to give a separate one (such as the separate descriptions of each kind of step above).}

We can represent the transition rules as Horn clauses, using the relation $R : S \to (M^*)^n\to o$ and the background theory in which $\le$ is the subword order on $M^*$ and $\cdot$ is string concatenation.


$\bullet$ If each $c_i$ is $u_i$ with some messages dropped, the state $(q_s,\bar{c})$ is reachable from the initial configuration $k_s=(q_s,\bar{u})$.

$$R\; q_s \bar{c} \impliedby \bigwedge_{i\in\{1,\ldots n\}} c_i\le u_i$$

$\bullet$ If a configuration $(q,\bar{c})$ is reachable from $k_s$, and $(q,i,?,a,q')\in \Delta$, and after dropping some messages and removing $a$ from the left, $c_i$ leaves $a\cdot c'$, then $(q',c_1\cdots c_{i-1}, c', c_{i+1}\cdots c_{n})$ is reachable from $k_s$.
$$R\; q'\; c_1\cdots c_{i-1}\; c'\; c_{i+1}\cdots c_{n} \impliedby R\; q\; \bar{c} \land a\cdot c' \le c_i$$

$\bullet$ If a configuration $(q,\bar{c})$ is reachable from $k_s$, and $(q,i,!,a,q')\in \Delta$, and after appending $a$ to the right and dropping some messages, $c_i$ leaves $c'$, then $(q',c_1\cdots c_{i-1}, c', c_{i+1}\cdots c_{n})$ is reachable from $k_s$.
$$R\; q'\; c_1\cdots c_{i-1}\; c'\; c_{i+1}\cdots c_{n} \impliedby R\; q\; \bar{c} \land  c' \le c_i \cdot a$$

We add a goal clause $false \impliedby R\; q_f\; \bar{u_f}$, leaving a system of clauses which is satisfiable if and only if $(q_f, \bar{u_f})$ is not reachable from $k_s$.

$$------------$$

\tcb{Original version below, it uses complementary definitions}


\tcb{For the moment, this section is notes.} 

\lo{@Toby: A decidability result building on this would be a really nice application.
	Lossy channel systems are studied in the more general context of WSTS in \cite{DBLP:journals/tcs/FinkelS01}, where several decidability results, including coverability (or control-state reachability) and termination, are presented.
	
	QUESTION: Can some of these results (or, better, decidability of new decision problems) be proved using initial limit datalog?}
\tcb{Yes. Specifically, below I've sketched a proof that the reachability problem for lossy channel systems is decidable. I will look more closely at the definition of WSTS to see how that compares to what I've shown here.}

\lo{QUESTION: If I am not mistaken, you need only 1st-order CHC for the present analysis of LCS. Use higher-order CHC to express an interesting decision problem.}
\tcb{You are correct. Since this is not a straightforward application of \cref{thm:order-main-sat-result}, it would take some care to mix higher-order clauses in. It would be possible - the hard part (testing validity of a model) only cares about decidabilty of individual clauses, so it is perfectly safe to add some extra higher-order clauses that make use of the reachability properties is fine. Mixing higher-order properties into the transition conditions might also be interesting, although it's not easy to see how initial higher-order clauses can be used to express properties that aren't obviously first order. }

\lo{QUESTION: There are connections with \Cref{thm:kuske and zetzsche} \cite{DBLP:conf/fossacs/KuskeZ19}.
	One could ask the preceding question, with the background theory set to the first-order theory of some bounded context-free language.}
\tcb{Could you clarify what you mean by "the preceding question, with the background theory set to the first-order theory of some bounded context-free language". Note that that theorem does not allow the use of constants which causes us some problems. (We need constants to express lower bounds)}

\newcommand{\lowercover}{\mathbin{\sqsupset\!\!\!\!\!\cdot\,}}
Lossy channel systems are a bit like lossy counter systems, but in place of counters, they make use of channels. 
There may be $m$ machines operating at once and they can communicate by either writing to or reading from a channel.

Questions about lossy channel systems can also be expressed as higher-order Horn clause problems. The clauses needed have the following forms:\tcb{First clause is for reading from a channel, second is for writing, The formal details should be obvious, but we can add them if we decide to keep this section.}
\lo{@Toby: Can you please briefly define LCS, and explain the following clauses?}
\lo{LCSs with multiple agents are equivalent with LCSs with a single agent. I would use the later.}


\begin{align*}
	R\; \bar{q}\; \bar{c} \impliedby R\; \bar{q'}\; \bar{c'} \land a\cdot c_{n+1}\le c_i \\ %reading
	R\; \bar{q}\; \bar{c} \impliedby R\; \bar{q'}\; \bar{c'} \land c_{n+1}\le c_i\cdot a \\ %writing
	R\; \bar{q_f}\; \bar{c} \impliedby \mathsf{true} %terminal
\end{align*}
where $$q'_j = \begin{cases}
	q_j \mathrm{\ if\ } j\ne k\\
	q' \mathrm{\ if\ } j = k
\end{cases}$$
$$c'_j = \begin{cases}
	c_j \mathrm{\ if\ } j\ne i\\
	c_{n+1} \mathrm{\ if\ } j = i
\end{cases}$$

$R\;\bar{q}\;\bar{c}$ should be true in the canonical model of these clauses if the state vector $\bar{q_f}$ is reachable from the states $\bar{q}$ with the channels holding the values in $\bar{c}$. Here, we are working in the theory of finite strings from a finite alphabet with $\le$ being the subword relation. States $q$ come from a finite set. \tcb{Technically we care about the theory of $n$-tuples of finite strings where $n$ is the number of channels.}

These are nearly limit Datalog problems, but the theory of strings under the subword ordering does not quite meet the requirement of decidability (It is a well-ordering, so there's some hope that this works). To get interesting results, we must more carefully examine the places in the proof where decidability is required.

The predicates used are $a\cdot x\le y$ and $x \le y \cdot a$ where $\le$ is the subword relation, $\cdot$ is concatenation and $a$ is a constant string. %Note that if we had both $x\le a\cdot y$ and $a\cdot y\le x$, we would be able to express $x=a\cdot y$. (true, but seems irrelevant)

%We can express upsets with these predicates - $\exists y.a\cdot y\le x$ is equivalent to $a\le x$,  but things are easier if we just add it to the language .

%but we might need to be careful about whether that looks like a universal quantifier when it's embedded in a clause (in the constructed clause, this appears on both sides of the implication). To make

To find a resolution proof of $\bot$ if one exists, we only need semidecidability of existential formulas. This is trivial because the space of words is countable and each background predicate is computable on concrete instances, so we can just try everything. \tcb{(According to \cite{DBLP:conf/lics/HalfonSZ17}, the existential fragment is not completely decidable when constants are involved, but that does not directly apply here.)}

For the other direction, we must examine the formulas constructed in \cref{lem:order-decidablemodel}. In this case, we begin with a formula of the form $R\; \bar{q}\; \bar{c} \impliedby R\; \bar{q'}\; \bar{c'} \land a\cdot c'\le c_i$. The states are from a finite set, so we may ground them and ignore them (like in the previous example). This leaves us with $\forall \bar{c}\ c'. R\; \bar{c} \impliedby R\; \bar{c'} \land a\cdot c'\le c_i$. The transformation process replaces predicates by descriptions of upsets (since we're working with a WQO, upsets can be specified as as described in \cref{sec:ldz} - a disjunction of terms of the form $a\le c_j$). 
\tcb{I'll quickly go through the transformation into something easy and neaten it up later}

\[\begin{array}{l}
	\forall \bar{c}\ c_{n+1}. R\; \bar{c} \impliedby R\; \bar{c'} \land a\cdot c_{n+1}\le c_i
	\\\forall \bar{c}\ c_{n+1}. R\; \bar{c} \lor \lnot R\; \bar{c'} \lor \lnot a\cdot c_{n+1}\le c_i
	\\\forall \bar{c}\ c_{n+1}. R\; \bar{c} \lor \lnot R\; \bar{c'} \lor \lnot a\cdot c_{n+1}\le c_i
	\\\forall \bar{c}\ c_{n+1}.\lnot (\lnot R\; \bar{c} \land  R\; \bar{c'} \land a\cdot c_{n+1}\le c_i)
	\\\lnot\exists\bar{c}\ c_{n+1}.\lnot R\; \bar{c} \land  R\; \bar{c'} \land a\cdot c_{n+1}\le c_i
\end{array}\]
We now apply the transformation. $\phi$ is some boolean combination of formulas of shape $a\le c$.
\[\begin{array}{l}
	\lnot\exists \bar{c}\ c_{n+1}. \phi \land a\cdot c_{n+1}\le c_i
	\\\lnot\exists \bar{c}\ c_{n+1}. (\bigvee\bigwedge \pm a\le c) \land a\cdot c_{n+1}\le c_i \textrm{\quad write $\phi$ in dnf}
	\\\lnot\bigvee\exists \bar{c}\ c_{n+1}. (\bigwedge \pm a\le c) \land a\cdot c_{n+1}\le c_i \textrm{\quad distribute and pull out}
	\\\lnot\bigvee\exists \bar{c}\ c_{n+1}. (\bigvee a^*\le c_{n+1}\land \bigwedge \pm a\le c) \land a\cdot c_{n+1}\le c_i
	\\\lnot\bigvee\bigvee\exists \bar{c}\ c_{n+1}.  a^*\le c_{n+1}\land (\bigwedge \pm a\le c) \land a\cdot c_{n+1}\le c_i
\end{array}\]
To reach the fourth line in the above, we note that since the space is a WQO, any upset can be written as a disjunction of lower bounds. In this case, we use the upset given by the conjunction of lower bounds on $c_{n+1}$. The expressions $\bigwedge \pm a\le c$ in the last 2 formulas do not contain $c_{n+1}$ negatively.

At this point, if we can decide $\exists \bar{c}\ c_{n+1}.  a^*\le c_{n+1}\land (\bigwedge \pm a\le c) \land a\cdot c_{n+1}\le c_i$, we are done. Since all predicates involving $c_{n+1}$ other than $a^*\le c_{n+1}$ are either upper bounds or negated lower bounds (if they hold at $c_{n+1}=k$ then they hold at $c_{n+1}$), if the formula holds, it holds when $c_{n+1}=a$. This leaves us with $\exists \bar{c}.  (\bigwedge \pm a\le c) \land a\cdot a^*\le c_i$ (assuming there were no contradictions which caused the formula to be false). Repeating the strategy used for $c_{n+1}$ for each $c_j$ in turn allows us to decide this formula.

The only properties we really needed here were that the subword relation is a WQO, that the transformation from an upset expressed as a conjunction into an upset expressed as a disjunction is computable, that the space of words is countable, that the background theory formulas used are computable on concrete instances and that concatenation with $a$ is monotone. This leads us to a few easy modifications which retain decidability - processes may be allowed to read or write from either end of a channel; (lossy channels of lossy counters ?) It looks like we're reaching the territory of well structured transition systems \cite{DBLP:journals/tcs/FinkelS01}. %\href{https://arxiv.org/abs/1301.5500}{The Power of Priority Channel Systems}  has already given results very similar to these (see the section on well-structured transition systems)

There's one last tricky bit I've missed - when considering clauses derived from writes, you're left with something of the shape $\exists c_i.  (\bigwedge \pm a\le c_i) \land a^*\le c_i\cdot a$. We can solve this by noting that $a^*\le c_i\cdot a \equiv a^{**}\le c_i$ where $a^{**}$ is $a^*$ with the longest suffix that's a substring of $a$ removed. In general, however, we need another condition - that the transformation of $a\le f(c)$ into a disjunction of lower bounds on $c$ is computable.

\tcb{I still need to check this more carefully (as well as write it up neatly)}
%A relevant result is \cite{DBLP:conf/lics/HalfonSZ17} which shows that we cannot allow all constants. Since $a\le x\land not(\bigvee_{b\lowercover\, a} b\le x)$ is equivalent to $x=a$, meaning that the fragment we care about is not decidable.

%\tcb{Since the questions we care about are decidable, we know that the systems of Horn clauses which answer these questions must also be decidable; but we'd like to use our proofs to show that this works}

One thing this tells us is that this proof method has very bad complexity bounds, since the reachability problem for lossy channel systems is complete for a ridiculous complexity class.

==> resource-example.tex <==
In the following example, we use higher-order clauses to model a set of keys in a way which is natural and yet retains decidability (which would be lost when modelling the same program using first-order Horn clauses over a general theory of lists or trees \cite{abiteboul-et-al-icdt13}).

\begin{example}[Resource Bound Analysis]
	\label{eg:resource bound}
	The following program implements a search for a data item $d$ in a finite-domain key-value store \cite{davoudian-et-al-acm-comp-surv-2018}.  The value obtained from one key determines the next key using some (unspecified)  logic.
	\begin{lstlisting}
	search : (Key -> Bool) -> Key -> Bool
	search seen k = if seen k then False else
							let v = query k in
								if v = d then True else
								let k' = logic v in search seen k'
	\end{lstlisting}
	Access to the store may be charged by the provider per query, so it is desirable to know that the number of queries is bounded by, for example, the number of keys in the store, say $K$.
	\begin{figure*}
		\iffalse
		$
		\begin{array}{r}
			\mathit{seen}\ k\ \mathsf{True} \wedge n = 0 \wedge b = False \to \mathrm{Search}\ n\ \mathit{seen}\ k\ b \\
			\mathit{seen}\ k\ \mathsf{False} \wedge \mathrm{Query}\ k\ d \wedge b = \mathsf{True} \wedge n = 1 \to \mathrm{Search}\ n\ \mathit{seen}\ k\ b \\
			\mathit{seen}\ k\ \mathsf{False} \wedge \mathrm{Query}\ k\ v \wedge v \neq d \wedge \mathrm{Logic}\ v\ k' \wedge \mathrm{Search}\ m\ \mathit{seen}\ k'\ b \wedge n = m + 1 \to \mathrm{Search}\ n\ \mathit{seen}\ k\ b \\
			b=\mathsf{False} \to \mathrm{Empty}\ k\ b\\
			\mathrm{Search}\ n\ \mathrm{Empty}\ k\ b \to n \leq K
		\end{array}
		$
		\fi
		\begin{align*}
			\mathrm{Search} &: \mathbb{Z} \to (\mathit{Key} \to \mathit{Bool} \to o) \to \mathit{Key} \to \mathit{Bool} \to o
			\\	
			\mathrm{Search}\, n\, \mathit{seen}\, k\, b
			& \impliedby 
			\mathit{seen}\, k\, \mathsf{True} \wedge n = 0 \wedge b = \mathsf{False} \\
			\mathrm{Search}\, n\, \mathit{seen}\, k\, b
			& \impliedby 
			\mathit{seen}\, k\, \mathsf{False} \wedge \mathrm{Query}\, k\, d \wedge b = \mathsf{True} \wedge n = 1
			\\
			\mathrm{Search}\, n\, \mathit{seen}\, k\, b
			& \impliedby 
		\mathit{seen}\, k\, \mathsf{False} \wedge \mathrm{Query}\, k\, v \wedge v \neq d \wedge \mathrm{Logic}\, v\, k' \wedge \mathrm{Search}\, m\, \mathit{seen}\, k'\, b \wedge n = m + 1\\
		\mathrm{Search}\, n\, \mathit{seen}\, k\, b
			& \impliedby 
			n=0 \\
			\mathrm{Empty}\, k\, b
			& \impliedby 
			b=\mathsf{False} \\
			n \leq K
			& \impliedby 
			\mathrm{Search}\, n\, \mathrm{Empty}\, k\, b
		\end{align*}
		\caption{Verifying accesses to the key-value store are bounded.}\label{fig:kv-example}
	\end{figure*}

	The situation can be formalised by the clauses in \cref{fig:kv-example}.
	The first three definite clauses capture the input-output behaviour of \lstinline{search} through the predicate $\mathrm{Search}$,
	with an additional integer parameter, $n$, that counts the number of queries.
	The purpose of the fourth clause is to provide a base case for this counting.
	The clauses are designed so that $\mathrm{Search}\, n\, \mathrm{Empty}\, k\, b$ is true in the least model just if there is a finite trace of the program in which $n$ queries are made.
	The goal clause asserts that accesses are bounded by the integer constant $K$.
	We assume that the behaviour of \lstinline{query} and \lstinline{logic} are overapproximated by definite clauses $\mathrm{Query}\,k\,v$ and $\mathrm{Logic}\,v\,k$.
	% The predicate $\mathrm{Search}$ has an interpretation modulo the theory of linear integer arithmetic (and the finite datatypes of keys, values and booleans) that satisfies the clauses just if the implementation satisfies the required property.
	
		The clauses are unsatisfiable (modulo the background theory, assuming a non-trivial set of data items) because the program has a bug: the \lstinline{seen} predicate is not updated in the recursive call.
		% Consequently, there is no integral bound on the number of resource accesses and execution of the program would get its author into serious financial difficulties.
		Fixing the program corresponds to adding to the following clause:
			%  representing the update of a finite map $m$ from keys to booleans by adding an additional key $k$:
		\changed[lo]{
		\begin{align*}
			\mathrm{Update}\, m\, k'\, k\, b
			& \impliedby
			(k = k' \wedge b = \mathsf{True}) \vee (k \neq k' \wedge m\, k\, b) %\to \mathrm{Update}\ m\ k\ k'\ b
		\end{align*}
		} \lo{Added brackets and swapped $k$ and $k'$ (to correspond to the replacement for $\mathit{seen}$).}
		and then replacing the offending $\mathit{seen}$ with $\mathrm{Update}\, \mathit{seen}\, k'$.
		This renders the modified system of clauses satisfiable.
\end{example}
